Toward Standardized Classification of Foveated Displays

Emergent in the field of head mounted display design is a desire to leverage the limitations of the human visual system to reduce the computation, communication, and display workload in power and form-factor constrained systems. Fundamental to this reduced workload is the ability to match display resolution to the acuity of the human visual system, along with a resulting need to follow the gaze of the eye as it moves, a process referred to as foveation. A display that moves its content along with the eye may be called a Foveated Display, though this term is also commonly used to describe displays with non-uniform resolution that attempt to mimic human visual acuity. We therefore recommend a definition for the term Foveated Display that accepts both of these interpretations. Furthermore, we include a simplified model for human visual Acuity Distribution Functions (ADFs) at various levels of visual acuity, across wide fields of view and propose comparison of this ADF with the Resolution Distribution Function of a foveated display for evaluation of its resolution at a particular gaze direction. We also provide a taxonomy to allow the field to meaningfully compare and contrast various aspects of foveated displays in a display and optical technology-agnostic manner.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> old_taxonomy.tex <==
% THIS IS THE OLDER 4-category characterization
% In order to describe these assumptions, we propose 4 elements that could be applied to all classes of foveated display.
% \begin{enumerate}
% \itemsep0em 
% \item Foveal Resolution
% \item Foveation Accuracy
% \item Resolution Distribution Function
% \item Effective Acuity Distribution Function
% \end{enumerate}

% \subsection{Foveal Resolution}
% We adopt the standard approach for human vision in describing the Foveal Resolution. That is, a nominal human visual acuity would be matched when the foveal resolution matches 20/20 (or 6/6 internationally). A display that only achieves half the acuity would be described as 20/40. Note that most readable content is designed to work for people with 20/40 vision, thus 20/40 acuity may be a good goal for foveated display designs.

% Let the \textbf{Acuity Ratio} be defined as the usual ratio used to represent visual acuity. For example someone with 20/20 vision would have an acuity ration of 1, while someone with 20/40 vision would have an acuity ratio of 0.5.

% Since is often useful to convert between different units, a simple conversion to pixels per degree ($\mathit{ppd}$) can be done with Equation~\ref{eqn:visiontoppd}. Equation~\ref{eqn:visiontoppi} shows how to convert from visual acuity to pixels per inch ($\mathit{ppi}$) at a distance of \emph{D} inches.

% \begin{equation}
% Resolution_{ppd} = 120\mathit{ppd} \times \mathit{AcuityRatio}
% \label{eqn:visiontoppd}
% \end{equation}
% \begin{equation}
% Resolution_{ppi} = \frac{1}{D \tan(\frac{1}{2 \mathit{ppd}})}
% \label{eqn:visiontoppi}
% \end{equation}

% \subsection{Foveation Error}
% Let us define \emph{foveation error} as the maximum angular distance between the central optical axis of the eye and the central optical axis of the display, particularly the region of foveal acuity. Foveation error can be thought of as the instantaneous difference between the ideal display position and actual display position given a user's gaze direction.

% Foveation error can arise from a number of sources including:
% \begin{itemize}
% \item Error in reported user gaze direction
% \item Error/speed/accuracy limitations of foveal steering mechanisms
% \item Latency in the adaptation of a display to updated user gaze direction
% \end{itemize}

% There are a variety of ways that one might measure the error of foveation for a display. Some possibilities include visual angle (degrees or radians), latency (seconds), or distance in display space (pixels). While each of these and other measurements could be useful for particular purposes, we suggest that visual angle is the most useful for classifying a foveated display.

% Given a display with a fixed size foveal region, the foveation error can be treated as an uncertainty region that needs to be removed from the total foveal field of view before reporting the achieved foveal region size. Alternatively, given a target foveal region field of view, this region needs to be increased in size by the foveation error to be able to guarantee the required foveal field of view.

% \todo[inline]{TODO Josef: add a figure to show this and how the fovea is effectively reduced in size due to reduced accuracy}

% \subsection{Resolution Distribution Function}
% The Resolution Distribution Function (RDF) describes the spatial/angular resolution presented by the display as a function of eccentricity, or angular displacement from the central optical axis of the display. 

% This is by far the most complicated aspect of classifying foveated displays in general. However, if we make an assumption that we are only interested in the maximum guaranteed resolution across the field of view of the display, and that the resolution is strictly decreasing with eccentricity, we can describe the resolution distribution function as a monotonic function of the eccentricity of the display. While this does not correctly match the human visual system which varies in acuity based on which radial angle is selected, and includes things like the blind spot, this does give us an effective way to classify displays by approximating the Acuity Distribution Function (ADF).

% One such approximation is the following function:

% \begin{equation}
% \frac{\partial r}{\partial \epsilon} = \begin{cases}
%     \dfrac{1}{F}, & \epsilon <= \epsilon_c \\
%     \dfrac{1}{S (\epsilon-\epsilon_0)}, & \epsilon > \epsilon_c
% \end{cases},
% \end{equation}

% When visualized with reasonable constants for 20/20 visual acuity, this function generates the chart in Figure~\ref{fig:acuity2020}.

% \begin{figure}
% \includegraphics[width=\columnwidth]{acuity2020}
% \caption{20/20 Visual Acuity Resolution Distribution Function}
% \label{fig:acuity2020}
% \end{figure}

% A display is said to be \emph{acuity matched} to a particular level of human visual acuity (i.e. 20/20 acuity matched) when its RDF exceeds a specified ADF over the entire display area. In order to further discuss this concept, it may be useful to examine an example.

% \todo[inline]{TODO Ben/Josef: Consider structuring an example, maybe put the example in a supplement or the discussion section at the end}

% \subsection{Stationary Foveated Displays}
% A stationary foveated display is one which does not attempt to change its resolution distribution function over time. This means the display cannot adapt to user conditions (such as gaze direction) beyond translating a region of uniform resolution (i.e. via soft steering).

% \subsection{Moving Foveation}
% Moving foveated displays are displays in which the display resolution distribution function changes over time. This may be accomplished via either hard or soft steering (or a mix of the two). Moving foveated displays require lower pixel counts than their (equivalent resolution) stationary alternatives as they are able to alter their resolution distribution function to align their highest resolution regions with the user's AOI.

% For the purpose of this work moving foveated displays will be subdivided into two further categories, \emph{moving inset displays} and \emph{fully moving displays}.

% \subsubsection{Moving Inset Displays}
% A moving inset foveated display maintains a fixed peripheral view (from the user's perspective) and (either hard or soft) steers only a sub-portion of the display (foveal inset) within this view. The peripheral view may be variable masked (i.e. soft steered) to register the inset, but the defining characteristic of moving inset displays is that the peripheral view display cannot be steered along with the inset. This operation is depicted in Figure \ref{fig:Moving_Inset_Single}. 

% \begin{figure}
% \includegraphics[width=\columnwidth]{Moving_Inset_Single}
% \caption{Demonstration of moving inset display showing peripheral view held constant while inset moves within the view}
% \label{fig:Moving_Inset_Single}
% \end{figure}

% \subsubsection{Fully Moving Displays}
% A fully moving display moves both the periphery and the inset jointly to maintain some relationship of the inset view to the peripheral field of view. This means the inset can either be maintained at the center of the periphery, or allowed to move within it according to some predetermined relationship. The ability to (hard or soft) steer both the periphery and the inset (not necessarily independent of one another) differentiates a fully moving display from a moving inset display. This is demonstrated in Figure \ref{fig:Fully_Moving_Single}.

% \begin{figure}
% \includegraphics[width=\columnwidth]{Fully_Moving_Single}
% \caption{Demonstration of fully moving display showing both peripheral view and inset moving together}
% \label{fig:Fully_Moving_Single}
% \end{figure}

% THIS IS THE OLD (RESOLUTION-ONLY) TAXONOMY, COULD PROBABLY BE REMOVED
%\subsection{Class I: Fully Foveated Displays}
%A Class I, or fully foveated display is the most complete class of foveation achievable by a display. When being viewed there is no perceivable roll-off in resolution over the full field of view at all possible viewing directions within the display.

%This implies that, at all possible gaze directions within its subtended view, a Class I foveated display has:
%\begin{itemize}
%\item Resolution meeting or exceeding the acuity of the user over the full field 5of view
%\item Imperceptible foveation error
%\end{itemize}

%As mentioned previously the bias of the user classifying the system is inherently included in the observation here. For this reason it is recommended that a Class I classification always come with the maximum visual acuity at which the claim has been validated (i.e. a Class I (20/30) Foveated Display).

%The simplest example of a Class I foveated display is an ultra-high resolution display placed sufficiently far from a user that the angular resolution exceeds the maximum visual acuity of most humans. This display meets all the criteria above for any point in its (albeit possibly small) active area and is therefore deemed a Class I foveated display.

% \subsection{Class II: Partially Foveated Displays}
% A Class II, or partially foveated display, is a Class I display in which the display RDF does not exceed the visual acuity of the user for the entire displayed field of view.

% Class II displays are separated into two subclasses to help better separate them by their limitations. Displays are separated into those that fail to exceed the (peak) foveal acuity of the user and those that provide other unpleasant effects due to mismatches between RDF and ADF.

% Class II displays can be thoroughly tested by visualizing a Snellen eye chart at various positions throughout the display with correct sizing. If the user is capable of performing an eye test at their nominal acuity then the display is acuity matched in the fovea. In the field this can also be quickly evaluated by examining detailed contents of a scene from variable distance/angle after observing them more closely to gain an understanding of their features.

% \subsubsection{Class 2a Foveated Displays}
% In a Class 2a, or hypo-resolution, display the foveal inset resolution does not exceed the visual acuity of the user for at least one static gaze direction. This could be due to insufficient optical performance or limited pixel pitch within the display. 

% Note that a Class 2a display must \emph{only be limited in peak foveal resolution}. This may become hard to delineate from Class 2b displays where lack of foveal region resolution may be perceived of in the far fovea/near periphery. Generally speaking, if the foveal resolution is sufficiently low to be perceived of in the periphery at all the display may be considered Class 2b rather than Class 2a.

% \subsubsection{Class 2b Foveated Displays}
% A Class 2b, or noticeably foveated, display may not qualify as Class 2a (if it does see Class III), but instead presents foveation artifacts that are visible to the user outside the foveal region. These effects are due to the user's visual acuity distribution exceeding the RDF at points other than the center of the foveal region of the display. This may result in tunnel-vision, peripheral flicker, or color separation in the near periphery.

% There are many more reasons a display may qualify as Class 2b than Class 2a. Some examples are provided below:
% \begin{itemize}
% \itemsep0em
% \item Undersized foveal region
% \item Undersized blend region
% \item Under approximated foveation error
% \item Over aggressive peripheral display resolution roll off
% \end {itemize}

% \todo[inline]{Someone w/ more knowledge of optics/perception should probably help validate this/fill this out}

% \subsection{Class III: Marginally Foveated Displays}
% A Class III, or marginally, foveated, display is a display which both fails to meet foveal acuity and introduces artifacts beyond the fovea (a display that is both Class 2a and Class 2b is considered Class III). This class of display encompasses everything from displays which may both fail to meet foveal acuity and peripheral resolution requirements simultaneously to systems that employ barrel distortion (where the perceived RDF is near the inverse of the model proposed in this work).

% Interestingly, modern VR systems should be considered Class III devices as they fail to meet foveal resolution (even at say 20/60 acuity) and tend to use lenses that impart barrel distortion as an unintended consequence of relocating the virtual image of the display to a comfortable viewing distance. In addition, since most VR systems don't steer this lens, the user sees lens astigmatism whenever their eye deviates from the position affiliated with the center of the lens/field of view.

% \begin{figure}
% \includegraphics[width=\columnwidth]{res4x}
% \caption{Visual Acuity Resolution Distribution Functions across different classes}
% \label{fig:res4x}
% \end{figure}

% We attempt to place all foveated displays into a set of classes based on how well they approximate the ideal foveated display, which would provide a high enough quality of visual output such that it is imperceptibly different from natural light. We use lower numbers to indicate that type of display is closer to ideal, while larger numbers indicate deviation from the idea to varying degrees. 

% \subsection{Type 1}
% A \textbf{Type 1} foveated display is one that meets or exceeds human visual acuity for a specified maximum foveal visual acuity. For example, a \emph{Type 1 20/20 Foveated Display} would indicate a display that produces images that are imperceptibly different from reality for a user with 20/20 visual acuity as measure by standard eye exams. 

% \subsection{Type 2}
% A \textbf{Type 2} foveated display is one that fails to match human perception in one way. In order to explicitly describe which kind of perception is not matched, we add a letter to the type as follows.

% \textbf{Type 2a:} This type of display moves as the user foveates, but does not attempt to directly match the visual acuity function with varying eccentricity. As an example, an inset display with a regular (or relatively regular) pixel grid which moves along with the gaze direction would be considered a Type 2a Foveated Display.

% \textbf{Type 2b:} This type of display attempts to match the visual acuity function with varying eccentricity, but does not move along with the gaze direction. One example would be a display with a regular pixel grid, which is then passed through some optical system which produces the perception of an irregular pixel distribution such as the one see in Figure~\ref{fig:type2b}.

% \subsection{Type 3}
% A Type 3 foveated display is one that does not particularly attempt to match human perception in the ways described as applying to foveated displays in general. While it may seem 

% \textbf{Visual Acuity Function Display:} Human visual acuity follows a certain function that can be approximated by a high angular resolution region in the center of vision with a falloff function similar to the one in Figure~\ref{fig:acuity}. Since not all humans achieve the same maximum visual acuity, we recommend describing such \emph{visual acuity function displays} by their maximum acuity as 20/20, 20/40, or whatever is appropriate for non-imperial parts of the world (6/6, 6/12, etc.).
